BridgeNets: Student-Teacher Transfer Learning Based on Recursive Neural Networks and its Application to Distant Speech Recognition

Despite the remarkable progress achieved on automatic speech recognition, recognizing far-field speeches mixed with various noise sources is still a challenging task. In this paper, we introduce novel student-teacher transfer learning, BridgeNet which can provide a solution to improve distant speech recognition. There are two key features in BridgeNet. First, BridgeNet extends traditional student-teacher frameworks by providing multiple hints from a teacher network. Hints are not limited to the soft labels from a teacher network. Teacher's intermediate feature representations can better guide a student network to learn how to denoise or dereverberate noisy input. Second, the proposed recursive architecture in the BridgeNet can iteratively improve denoising and recognition performance. The experimental results of BridgeNet showed significant improvements in tackling the distant speech recognition problem, where it achieved up to 13.24% relative WER reductions on AMI corpus compared to a baseline neural network without teacher's hints.

==> BridgeNets_old.tex <==
\section{BridgeNets}
\label{sec:bridgenet}

\subsection{Recursive Architecture}
\label{sec:recursive}

In this section, we present a new recursive architecuture as a part of BridgeNets.
A recursive neural network is popularly used in sentence parsing, sentimental analysis,
sentence paraphrase detection and many other areas. It applies the same set of weights
recursively over a structure. Its concept is similar to a recurrent network but there is a clear
difference in that a recursive neural network can traverse a given structure in any topological order.

Figure~\ref{fig:recursive_a} (a) shows building blocks of a proposed recursive architecture.
It is composed of four blocks: $C^0$, $L_1^0$, $F^0$ and $L_2^0$. Upper subscripts indicate the number
of recursions. Each block can be any network. For example, $C^0$ can be a CNN network, whereas
$L_1^0$ or $L_2^0$ can be a LSTM network. $F^0$ combines two input paths: one is from an acoustic
input and the other is from the output of the prior recursion. $L_{init}$ is a zero
vector used as input for the zero recursion. 

The advantage of this sub-block division enables a network to recurse with heterogeneous input
and output types. For example, a typical acoustic model has context-dependent phones as a
network output. This output cannot be fed into an input for the next recursion because the network
input is an acoustic signal that is totally different from phone states. The proposed architecture
provides two different input paths. They are processed independently and combined later at $F^0$. 

Figure~\ref{fig:recursive_a} presents how to unroll the proposed recursive network in the depth
direction. $R$ implies the number of recursion. The same input $x_t$ is
applied to the network for each recursion. This repeated input acts as a global shortcut path
that is critical to train a deep architecture. Our proposed recursive network can be formulated
as follows:
\begin{equation}
\label{eq:recursive_0}
F^n = h\left( W_{1}C^{n} + W_{2}L_{1}^{n}\left( L_{2}^{n-1}\right) + b\right)
\end{equation}
$W_{1}$, $W_{2}$ and $b$ are internal parameters of $F^{n}$. Two paths are affine-transformed and
added together before going into nonlinear function $h$. Compared with the recursive residual
network proposed in~\cite{taiimage}, our model has two differences. First, the model in~\cite{taiimage}
can only recurse with homogeneous input and output. Second, global connection is always added
with the output of the prior recursion in~\cite{taiimage} but our model allows to flexibly
combine two heterogeneous inputs.
Simple addition is a special case of Eq.~\ref{eq:recursive_0}.

\begin{figure}[htb]
\begin{minipage}[b]{0.32\linewidth}
  \centering
  \centerline{\includegraphics[width=1.6cm]{figs/recursive_0_new-crop.pdf}}
%  \vspace{1.5cm}
  \centerline{(a) $R=0$ }\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.32\linewidth}
  \centering
  \centerline{\includegraphics[width=1.9cm]{figs/recursive_1_new-crop.pdf}}
%  \vspace{1.5cm}
  \centerline{(b) $R=1$}\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.32\linewidth}
  \centering
  \centerline{\includegraphics[width=2.2cm]{figs/recursive_2_new-crop.pdf}}
%  \vspace{1.5cm}
  \centerline{(c) $R=2$}\medskip
\end{minipage}
%
\caption{ Unrolling of a Recursive Network: $R$ is the number of recursions.
(a), (b) and (c) show how a recursive network is unrolled in the depth direction. The same
input $x_t$ is fed to a recursive network for each recursion, which acts as a global shortcut path.
The blocks with the same color share the same weights.}
\label{fig:recursive_a}
\end{figure}
\subsection{Network Description}
BridgeNet provides novel student-teacher transfer learning combined with a new recursive
architecture. Figure~\ref{fig:br_overview} presents a high-level block diagram of BridgeNet.
Both student and teacher networks are constructed from a recursive network.
They don't need to have the same recursions.
Typically, a teacher network can have more recursions because its complexity only matters
during training stage.

BridgeNet uses a collection of triplets as training data: $\left(x_t^*,x_t,y_t \right)$.
$x_t^*$ is enhanced or less noisy data, $x_t$ and $y_t$ are noisy data and their labels.
A teacher network is first trained with $x_t^*$ and $y_t$ pairs. 
Next, the trained teacher network provides its internal feature representations
as hints to a student network.
All connections between student and teacher networks are defined as knowledge bridges.
An error measure $e_i$ of how a feature representation $q_i$ from a student network agrees
with the hint $h_i$ is computed at the knowledge bridge as a MSE loss.
\begin{equation}
e_{i}(\phi_S) = \sum_{t=1}^{L}\left|h_{i}(x^{*}_{t})-q_{i}(x_{t};\phi_S)\right|^{2}
\label{eq:kb_1}
\end{equation}
Since $h_1$ and $q_1$ are softmax probabilites of teacher and student networks,
the cross-entropy loss is used for $e_1$ instead.
\begin{equation}
e_1(\phi_S) = -\sum_{t=1}^{L}P_{T}(x_{t}^{*};\phi_T)\log P_{S}(x_{t};\phi_S)
\end{equation}
The parameters of the student network are then optimized by minimizing a weighted
sum of all corresponding loss functions.
\begin{equation}
L(\phi_S) = \sum_{i=1}^{N}\alpha_{i} e_{i}(\phi_S)
\end{equation}
\begin{figure}[h]
  \centering
  \centerline{\includegraphics[width=7.0cm]{figs/bridgenet_recursive_diagram-crop.pdf}}
\caption{Conceptual Diagram of BridgeNet}
\label{fig:br_overview}
\end{figure}

Since student and teacher networks have multiple recursions, the same knowledge bridges can be
repeadtedly connected for each recursion.
However, any knowledge bridge in the intermediate recursion always degraded performance.
It is conjectured that feature representations at the last recursion would be the most relevant
and accurate to predicting correct phone states. Therefore,
BridgeNet adds knowledge bridges only at the last recursion as shown in Figure~\ref{fig:br_overview}.
%knowledge bridges only at the last recursion showed the best performance. Any additional
%knowledge bridge in the itermediate recursions always performs worse.
%It is conjectured that feature representations at the last recursion would be the most relevant
%and accurate to predicting correct phone states.

Figure~\ref{fig:cnn_lstm} shows our implementation of a recursive network for student
and teacher networks. As described in Section~\ref{sec:recursive}, it comprised of four
components: CNN layers ($C$), first LSTM layers ($L_1$), second LSTM layers ($L_2$) and
dimension reduction layer ($F$). Upper subscripts are omitted for simplicity. 

Since feedback phone states and acoustic input don't have
correlations in frequency and time directions, they cannot be fed into
the same CNN layers. Instead, feedback phones are separately processed in $L_1$ controlled
by a gate network, $g_n^{fb}$. Its formulation is referred from~\cite{chung2015gated},
\begin{equation}
g^{fb}_{n} = \sigma\left( w_x x_t + w_s s_{t,n-1} + w_{h} h_{t,n} \right)
\end{equation}
where $s_{t,n-1}$ is a feedback state from ${n-1}^{th}$ recursion, $h_{t,n}$ is
an $L_1$ output at $n^{th}$ recursion and $w_x$, $w_s$ and $w_h$ are weights to be learned.
Two input paths are combined
later at the dimension reduction layer. The dimension reduction layer is a fully-connected
one to merge them and reduce their dimensions for the second LSTM block, $L_2$.

A residual LSTM~\cite{kim2017residual} is used for $L_1$ and $L_2$ blocks.
It has a shortcut path between layers to avoid vanishing or exploding gradients commonly
happening to deep networks. It was shown that when a network depth gets deeper,
residual LSTM performs gredually better than plain LSTM.
\begin{figure}[h]
  \centering
  \centerline{\includegraphics[width=5.3cm]{figs/recursive_imp-crop.pdf}}
\caption{CNN-LSTM Recursive Network}
\label{fig:cnn_lstm}
\end{figure}

%Similar to Hinton's distillation~\cite{hinton2015distilling}, BridgeNet uses a well trained
%teacher network to provide soft targets to guide a student network. However, there are several
%key differences in BridgeNet. First, BridgeNet uses different data sets to train student
%and teacher networks. A teacher network is trained with enhanced or less noisy data
%, which was first proposed in ~\cite{lopez2015unifying,markov2016robust_1}.
%Second, BridgeNet further improves a student network with additional hints from a teacher's
%intermediate feature representations. We defined these hints connections as knowledge bridges.
%Finally, recursive architecture is combined with student-teacher framework. There have been
%many iterative approaches to get feedback from HMM states to further refine ASR performance.

%Three knowledge bridges are used for evaluation: Knowledge Distillation (KD) at
%the softmax output, LSTM3 at the last LSTM output of $L_2$ and DR
%at the output of the dimension reduction layer. 

%\subsection{Discussion on Related Works}

%DeepID~\cite{sun2015deeply,sun2015deepid3} presented a face verification network deploying Siamese twin networks  connected by
%verification supervisory signals at intermediate layers, One main difference, is that both networks share the same weights and are trained simultaneously on same data to make their intermediate representation closer when they have examples for the same identity or farther away for
%different identities. Hence, this does not fit the BridgeNet student-teacher paradigm where Teacher network is trained in advance on different data.
%FitNet~\cite{romero2014fitnets}
%uses a hint from a teacher's intermediate layer to train a thinner and deeper student network. Its
%concept is similar to BridgeNet but there are several differences. First, 



%The hint is used to separately train a student subnetwork to be used as a pretrained model for later
%fine tuning.

%when the student network is later fine-tuned independently. BridgeNet avoids such multi-step learning approach, by training the student network with all hints together by minimizing the weighted loss function as in multi-task learning. Moreover, when the student network is trying to learn a different function from a different data set other than that of the teacher  as in BridgeNet, this weight initialization process may not be beneficial.

%A knowledge sharing model \cite{qian2016investigation} has been proposed for distant speech.
%A close-talk network and a far-field network are linked together at intermediate connections for knowledge sharing. However, both networks are trained simultaneously, and gradients from a far-field network can influence a close-talk network or vice versa. Hence, this training strategy fits a peer-to-peer training paradigm rather than BridgeNet's student teacher paradigm.

%Furthermore, \cite{qian2016investigation} reported
%its performance is even worse than multi-task denoising that is shown to perform much worse than
%BridgeNet.




==> Related.tex <==
\section{Related Works}
\label{sec:related}


==> backup_Experiments.tex <==
\section{Experiments}
\subsection{Experimental Setup}

AMI corpus\cite{carletta2005ami} provides 100 hours meeting conversations
recorded with multiple microphones. Corpus recorded by individual headset microphones (IHM)
provides clean conversation with small interference or noise. Corpus by single distant
microphones (SDM) is noisy and corrupted by interference from other speakers. SDM corpus
can be enhanced by beamforming multiple channels, which is MDM corpus. In this paper,
IHM corpus is used to train a teacher network, and a student network is trained 
with SDM or MDM corpus.

Kaldi~\cite{Povey_ASRU2011} is used to train context-dependent GMM-HMM system. 
The trained GMM-HMM is used to generate forced aligned labels to train BridgeNet.
Since IHM and SDM corpora are synchronized, alignment labels generated by IHM corpus
are used to train both student and teacher networks.

Microsoft Cognitive Toolkit (CNTK)~\cite{yu2014introduction} is used to train and decode
BridgeNet. 
The DNN model evaluated in this paper has 8 layers with the same internal
structure as the joint-learning
model in\cite{qian2016investigation}. For BridgeNet, 
two convolutional layers in a
feature network have 9x9 and 3x1
filters with 256 feature maps.
80-dimensional log Mel filterbank features are generated as a feature vector and
9 frames of feature vectors are concatenated and fed into a feature network.
Each residual LSTM in a recognition network has 1024 memory cells and 512 hidden nodes.
The final softmax output has 3902 context-dependent phone classes. At later sections,
BridgeNet baseline model will be called CONV-LSTM for an efficient notation.

Since SDM or MDM corpus is a meeting conversation between multiple speakers,
we provides two types of word error rates (WER): Overlapped and non-overlapped WERs.
The overlapped WER is to decode up to 4 concurrent speeches, which
is a big challenge considering training procedure only focuses on a main
speaker. The non-overlapped WER is to decode single main speaker, which is
more realsitic performance measure for SDM or MDM corpus. We provides both WERs
in the later evaluations.

\subsection{Multi-Task Denoising on AMI Corpus}
\label{sec:multi}

Table\ref{tab:mtd} provides WER evaluation of multi-task denoising on SDM corpus.
Multi-task denoising shows only 0.7\% and 0.6\% non-overlapped WER reduction on DNN and
CONV-LSTM, which is contrary to the bigger improvement observed in~\cite{qian2016investigation}.
The main difference is that our DNN model showed significantly lower WER.
Improvement from multi-task denoising
looks decreasing with better performing acoustic model. To confirm this pattern,
CONV-LSTM is trained with clean alignments generated from IHM corpus. Non-overlapped WER
of CONV-LSTM got improved more
than 9\% simply changing alignment labels. However, multi-task denoising on the
improved CONV-LSTM degraded from 37.8\% to 38.2\%. 


\subsection{BridgeNets on AMI Corpus}
\label{sec:ex_br}
Table~\ref{tab:br_sdm} presented BridgeNet WER performance
for SDM corpus. The baseline
CONV-LSTM is trained without a teacher network.
KD is BridgeNet only with a knowledge distillation
connection described in Eq.~\ref{eq:kd}. 
KD+DR implies BridgeNet with two connections: knowledge distillation and
a knowledge bridge between dimension reduction layers.
Finally, KD+DR+LSTM3 is BridgeNet with all three connections described in Eq.~\ref{eq:bn}.

BridgeNet only with KD showed 2.1\% WER reduction over baseline model. With additional
knowledge bridges, KD+DR and KD+DR+LSTM3 showed 4.0\% and 5.9\% WER reduction over baseline
model, respectively. Compared with multi-task denoising which did not show any improvement
with clean alignment labels, BridgeNet continuously improves with additional bridge connections.
The main difference is to provide bridge connection with the same level of abstraction from a
teacher network, which proved to be more beneficial than directly using low-level clean features.

Table~\ref{tab:br_mdm} presented BridgeNet WER performance on MDM corpus. MDM corpus is
generated by beamforming 8 channel distant microphone recordings
using BeamformIt\cite{anguera2007acoustic}. Using MDM corpus, absolute WER decreased more
than 10\% compared with SDM corpus. BridgeNet, however, still provided similar improvements on
MDM corpus.
KD, KD+DR and KD+DR+LSTM3 provided 2.6\%, 4.4\% and 5.3\% WER reductions, respectively.


\begin{table}
\caption{Multi-Task Denoising on SDM: $\text{CONV-LSTM}^{*}$ was
trained with clean alignments from IHM. Other models used
noisy alignments from SDM}
\label{tab:mtd}
\vspace{0.2cm}
\centering
\begin{tabular}{l r r }
\toprule
 Acoustic Model   &  WER(over) & WER(non-over) \\
 \midrule
 DNN   & 59.1\% & 50.5\% \\
 DNN, denoised   & 58.7\% & 50.2\% \\
 CONV-LSTM  & 50.4\% & 41.6\% \\ 
 CONV-LSTM, denoised & 50.1\% & 41.4\%\\
 \midrule
$\text{CONV-LSTM}^{*}$ & 46.7\% & 37.8\%\\
$\text{CONV-LSTM}^{*}$, denoised& 46.9\% & 38.2\%\\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{BridgeNet Evaluation on SDM: All networks are trained with clean alignments.}
\label{tab:br_sdm}
\vspace{0.2cm}
\centering
\begin{tabular}{l r r }
\toprule
 Acoustic Model   &  WER(over) & WER(non-over) \\
 \midrule
 CONV-LSTM (Baseline)  & 46.7\% & 37.8\% \\
 KD   & 45.7\% & 37.0\% \\
 KD+DR  & 45.3\% & 36.3\% \\ 
 KD+DR+LSTM3 & 44.9\% & 35.7\% \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{BridgeNet Evaluation on MDM8: All networks are trained with clean alignments. }
\label{tab:br_mdm}
\vspace{0.2cm}
\centering
\begin{tabular}{l r r }
\toprule
 Acoustic Model   &  WER(over) & WER(non-over) \\
 \midrule
 CONV-LSTM (Baseline)   & 43.4\% & 34.0\% \\
 KD   & 42.8\% & 33.1\% \\
 KD+DR  & 42.3\% & 32.5\% \\ 
 KD+DR+LSTM3 & 41.8\% & 32.2\% \\
\bottomrule
\end{tabular}
\end{table}


==> backup_Related.tex <==
\section{Related Works}
\label{sec:method}
%In this section, we highlight several releated works. First, we review
%multi-task denoising which jointly optimizes denoising and recognition networks. Second,
%We describe student-teacher knowledge distillation learning. Finally, we explain
%curriculum transfer learning that incrementally train a network with augmented harder data.

\subsection{Multi-Task Denoising}
\label{sec:mtd}

Multi-task denoising~\cite{qian2016investigation,ravanelli2016batch}
was proposed to jointly optimize denoising and recognition networks integrated
within the unified neural network. The denoising network gets noisy
acoustic input $x^{noisy}_{t}$ at time $t$ and tries to reproduce denoised enhanced
feature $x^{de}_{t}$ by MSE regression with synchronized clean acoustic
input $x^{clean}_{t}$.
%\begin{equation}
\begin{eqnarray}
\label{eq1}
L_{mse}(W_{de}) &=& \sum^{T}_{t=1} \left|x^{de}_{t}-x^{clean}_{t}\right|^{2}
\end{eqnarray}
Where, $T$ is mini-batch size and $W_{de}$ is a collection of learnable
parameters in the denoising network.
The enhanced feature $x^{de}_{t}$ is fed into the recognition
network to predict phone sequences.
Since the denoising network is cascaded with the recognition network, gradients
from the recognition block are also back-propagated into the denoising parameters.
The final multi-task loss function can be described as follows.
\begin{equation}
L_{ce}(W_{de},W_{re})= \sum^{T}_{t=1} \text{CE}(y^{label}_{t},P(x^{de}_{t}) )
\end{equation}
\begin{equation}
L(W_{de},W_{re})= (1- \alpha) L_{ce}(W_{de},W_{re}) + \alpha L_{mse}(W_{de})
\end{equation}
where $W_{re}$ is a collection of learnable parameters in the recognition network,
$\text{CE}(\cdot,\cdot)$ is a cross-entropy, $P(\cdot)$ is the softmax output of the
recognition network, $y_{t}^{label}$ is a ground truth label at $t$  and
$\alpha$ is a weighting factor to balance between two loss functions.

%Multi-task denoising showed some improvements for the DNN architecture in
%\cite{qian2016investigation,ravanelli2016batch}, but
%the performance of convolutional LSTM architecture proposed in Figure~\ref{fig:br} degraded,
%which will be shown in Section~\ref{sec:multi}.

\subsection{Knowledge Distillation}
\label{sec:k_dist}
In knowledge distillation, a student network is trained by
a more general and bigger teacher network~\cite{hinton2015distilling,romero2014fitnets}.
The basic idea is to provide the additional
softmax output from a teacher network.
The student network, then, can capture subtle relation between ground truth and non-target
classes which would be difficult to obtain only from hard target labels.

Let $x_{t}^{noisy}$ be an input feature for both teacher and student networks at time $t$.
Then, $P_{T}(x_{t}^{noisy})$ is an softmax output of a teacher network and
$P_{S}(x_{t}^{noisy})$ is an softmax output of a student network.
Network outputs can be softer or
harder by parameterizing temperature parameter, $\tau$ as follows.
\begin{equation}
P_{T}=\text{softmax}(a_{T}/\tau), P_{S}=\text{softmax}(a_{S}/\tau)
\end{equation}
where $a_{T}$ and $a_{S}$ are input logits to softmax layers for teacher and student
networks, respectively. Input arguement $x_{t}^{noisy}$ is omitted for the efficient notation.
The student network is, in turn, trained to minimize the following loss function.
%\begin{equation}
\begin{eqnarray}
\label{eq:kd}
L_{KD}(W)&=&(1-\alpha)\sum_{t=1}^{T}CE(P_{T}(t), P_{S}(t)) + \nonumber \\
&&\alpha \sum_{t=1}^{T}CE(y_{t}^{label},P_{S}(t))
\end{eqnarray}
A teacher network is trained with the same training data
and applied to a smaller and compact student network for network compression
in \cite{hinton2015distilling,romero2014fitnets}.
The extended knowledge distillation
\cite{lopez2015unifying, markov2016robust_1, markov2016robust_2}
uses separate privileged data to a teacher network for better
posterior estimation.
In~\cite{markov2016robust_1, markov2016robust_2},
a teacher network is trained with parallel clean data instead
of noisy one. Through knowledge distillation, the teacher network can implicitly transfer
how to denoise noisy data in a student network.


\subsection{Curriculum Learning}
\label{sec:ctl}
Curriculum learning was proposed to find a better local minimum by incrementally training a
network with a predefined sequence of training data. The intuition is to train a network
from an easy data and then repeat training with augmented harder examples.
\cite{bengio2009curriculum} showed that a carefully chosen sequence of training data can
accelerate training convergence with better generalization performance. 
One example of a curriculum is to generate
a sequence of training data with increasing noise variance. A network is then trained from
less noisy data to more noisy one.
%which is similar to the concept of the extended
%knowledge distillation \cite{markov2016robust_1, markov2016robust_2}
%explained in Section~\ref{sec:k_dist}.
%One difference is that curriculum learning directly uses less noisy or easy data for
%training but the latter uses a higher level of feature representation from the trained teacher
%network.

